A mean-field limit for certain deep neural networks

Understanding deep neural networks (DNNs) is a key challenge in the theory of machine learning, with potential applications to the many fields where DNNs have been successfully used. This article presents a scaling limit for a DNN being trained by stochastic gradient descent. Our networks have a fixed (but arbitrary) number $L\geq 2$ of inner layers; $N\gg 1$ neurons per layer; full connections between layers; and fixed weights (or "random features" that are not trained) near the input and output. Our results describe the evolution of the DNN during training in the limit when $N\to +\infty$, which we relate to a mean field model of McKean-Vlasov type. Specifically, we show that network weights are approximated by certain "ideal particles" whose distribution and dependencies are described by the mean-field model. A key part of the proof is to show existence and uniqueness for our McKean-Vlasov problem, which does not seem to be amenable to existing theory. Our paper extends previous work on the $L=1$ case by Mei, Montanari and Nguyen; Rotskoff and Vanden-Eijnden; and Sirignano and Spiliopoulos. We also complement recent independent work on $L>1$ by Sirignano and Spiliopoulos (who consider a less natural scaling limit) and Nguyen (who nonrigorously derives similar results).

==> measureNN_aux/0-notation.tex <==
Given integers $a,b\in\Z$ with $a\leq b$, $[a:b]:=\Z\cup [a,b]$ is the set of all integers between (and including) $a$ and $b$.

Given a Polish space $(X,\rho_X)$, $\Probspace(X)$ is the set of probability measures over $X$. 

We use $|\cdot|$ to denote the Euclidean norm over some $\R^d$, $\|\cdot\|$ to denote the standard $2\to 2$ norm over linear transformations $\R^{d_1}\to\R^{d_2}$, and $\|\cdot\|_{\infty}$ to denote the supremum norm over continuous functions in $C([0,T],\R^{d})$ (for some $d\in\N$).





==> measureNN_aux/2-mkeanvlasov.tex <==
We now explain the mean-field behavior we expect from our system in the large-$N$ limit.

\subsection{An ansatz} The basic idea behind our model is that the summations appearing in the gradients of $L_N$ are to be replaced by integrals over conditional distributions. This idea was applied nonrigorously (and independently) by Nguyen \cite{Nguyen2019}. The {\em ansatz} can be summarized as follows:
\begin{itemize}
\item Weights on the same layer are statistically indistinguishable.
\item Gradients of weights in layers $\ell=0,1,2,3,\dots,L-1,L$ depend on averages taken over network paths. Some paths go "backwards" to the input and some go "forward" to the output.
\item Weights $\theta^{(\ell)}_{i_\ell,i_{\ell+1}}$ in layers $2\leq \ell\leq L-2$ have lots of paths both ways. If averages become deterministic integrals, we expect these weights to decouple from the rest of the network. The same holds for weights in layer $\ell=0$ (only forward paths) and $\ell=L$ (only backward paths).
\item By contrast, a weight $\theta^{(1)}_{i_1,i_{2}}$ has one backwards path through $\theta^{(0)}_{1,i_1}$. So we expect that $\theta^{(1)}_{i_1,i_{2}}$ will depend on $\theta^{(0)}_{1,i_{1}}$ (but will decouple from other weights) even in the thermodynamic limit. A similar reasoning shows that $\theta^{(L-1)}_{i_{L-1},i_{L}}$ should depend on $\theta^{(L)}_{i_L,1}$, but on no other weights.
\end{itemize}

This leads us to consider {\em input-to-output paths} in the network as our basic units in the analysis:
\begin{equation}\label{eq:defpath}
	\theta = \parn{\theta^{(0)}_{1,i_1},\theta^{(1)}_{i_1,i_2},\theta^{(2)}_{i_2,i_3},\dots,\theta^{(L)}_{i_L,i_1}}.
\end{equation}
Figure \ref{fig:unit} illustrates one such path.
\input{measureNN_aux/fig2-path}
If our ansatz is correct, understanding the distribution of weights on a path suffices to describe the law of all weights in the network. We clarify this in the next subsection. 

\subsection{Paths and measures} Note that the vector $\theta$ in (\ref{eq:defpath}) lives in
\begin{equation}
	\R^{D_0}\times \R^{D_1} \times \dots \times \R^{D_L}\cong \R^D\mbox{ ,where }D:= D_0 + D_1 + D_2 + \dots + D_L.
\end{equation}

Therefore, given $x\in \R^D$, we write $x= (x^{(\ell)})_{\ell=0}^L$ with each $x^{(\ell)}\in \R^{D_\ell}$. We will need some notation for the high-dimensional measures.

\begin{definition}[Marginals]
Let $\mu$ be a probability measure over $\R^{D}$. Given $i\in [0:L]$, we write $\mu^{(i)}$ to denote the marginal over the $i$-th factor $\R^{D_i}$ of the Cartesian product. That is, if $\Theta\sim \mu$, then $\Theta^{(i)}\sim \mu^{(i)}$. If $i\leq L-1$, we write $\mu^{(i,i+1)}$ for the marginal over the $i$-th and $(i+1)$-th factors. We also use the symbol $\mu^{(i\mid i+1)}(\cdot\mid a^{(i+1)})$ to denote the conditional distribution of $\Theta^{(i)}$ given $\Theta^{(i+1)}=a^{(i+1)}$.
\end{definition}

Note that the heuristic analysis suggests a factorization for the distribution over a path: the measure over a path should factor as
\begin{equation}\label{eq:mufactorizes}\mu = \mu^{(0,1)}\times \mu^{(2)}\times \dots \times \mu^{(L-2)}\times \mu^{(L-1,L)}.\end{equation}

Moreover, if we can compute the law of the weights on a path, the weights over the entire network should factor (approximately) as follows, at any fixed training step.
\begin{enumerate}
\item We expect $\theta^{(\ell)}_{i_\ell,i_{\ell+1}}\sim \mu^{(\ell)}$ independently for all $\ell\neq 1,L-1$ and $(i_\ell,i_{\ell+1})\in [1:N_\ell]\times [1:N_{\ell+1}]$.
\item Conditionally on the above choices, we expect that the weights on layers $\ell=1,L-1$ are conditionally independent, with $\theta^{(1)}_{i_1,i_2}\sim \mu^{(1\mid 0)}(\cdot\mid \theta^{(0)}_{1,i_1})$ and $\theta^{(L-1)}_{i_{L-1},i_L}\sim \mu^{(L-1\mid L)}(\cdot\mid \theta^{(L)}_{i_L,1})$.\end{enumerate}

We will eventually make this precise via the introduction of "ideal particles". It will be crucial that the above independence structure also works at the level of {\em trajectories}. For this we will need the following notation.

\begin{definition}[Measures on trajectories]
\label{def:measuresontraj}
We use symbols such as $\mu_{[0,T]}$ (greek letter with the subscript $[0,T]$) to denote a probability measure over the product space
\[
	C([0,T],\R^{D}) \cong \bigotimes_{i=0}^{L} C([0,T],\R^{D_i}).
\]
As in the previous definition, if $i\in[0:L]$, we write $\mu_{[0,T]}^{(i)}$ to denote the marginal over the $i^{\text{th}}$ factor in the above product (which is a probability measure over $C([0,T],\R^{D_i})$). Moreover, if $i\in[0:L-1]$, we write $\mu_{[0,T]}^{(i,i+1)}$ for the marginal over both $i^{\text{th}}$ and $(i+1)^{\text{th}}$ factors (which is a probability measure over $C([0,T],\R^{D_i}\times\R^{D_{i+1}})$). We also use $\mu^{(j\mid i)}_{[0,T]}(\cdot\mid x^{(i)}_{[0,T]})$ to denote the conditional distribution of the ($j$th) component given the $i$th component.  Also, we use a subscript $0\leq t\leq T$ to denote the marginal at time $t$, which is a probability measure over $\R^{D}$.

This means, for instance, that if $\Theta \sim \mu_{[0,T]}$, then $\mu_{t}$ is the law of $\Theta(t)$, $\mu^{(i)}_t$ is the law of its $i^{\text{th}}$ coordinate $\Theta^{(i)}(t)$, $\mu^{(i)}_{[0,T]}$ is the law of the $i^{\text{th}}$ coordinate's trajectory $\Theta^{(i)}\in C([0,T], \R^{D_i})$, and $\mu^{(j\mid i)}_{[0,T]}(\cdot\mid x^{(i)}_{[0,T]})$ is the law of $\Theta^{(j)}_{[0,T]}$ conditionally on $\Theta^{(i)}_{[0,T]}=x^{(i)}_{[0,T]}$.\end{definition}


\subsection{Mean-field representation of network evolution}
\label{sub:McKeanVlasov}
With our heuristic in mind, we define the "mean-field substitutes" for the function $\yhat$ and the gradients that will appear in the analysis. We first describe what happens when we apply our ansatz to approximate the terms $z^{(\ell)}_{i_\ell}$ (\ref{eq:defzell}) and $M^{(\ell)}_{\boldj{\ell}{L+1}}$ (\ref{eq:defM}) in the definition of gradients. The idea is that the summations will converge to integrals over factors of the measure $\mu$.
\subsubsection{The mean-field versions of the $z$'s.}
We consider a series of mappings taking as input a pair $(x,\mu)\in \R^{d_X}\times \Probspace(\R^D)$. We first define
\begin{equation}
\label{eq:defzbar2}
	\zbar^{(2)}(x,\mu):=
	\int\limits_{\R^{D_0}\times \R^{D_1}}\sigma^{(1)}\parn{\sigma^{(0)}(x,a^{(0)}),a^{(1)}}\,d\mu^{(0,1)}(a^{(0)},a^{(1)}).
\end{equation}

For $2<\ell\leq L-1$, we define:
\begin{equation}
\label{eq:defzbarell}
	\zbar^{(\ell)}(x,\mu):=
	\int\limits _{\R^{D_{\ell-1}}}\sigma^{(\ell-1)}\parn{\zbar^{(\ell-1)}(x,\mu),a^{(\ell-1)}}\,d\mu^{(\ell-1)}(a^{(\ell-1)}).
\end{equation}

The case of $\zbar^{(L)}$ is different: we define it in terms of $x$ and the {\em conditional distribution} $\mu^{(L-1\mid L)}$. Letting $a^{(L)}\in R^{D_L}$, we define:
\begin{equation}
\label{eq:defzbarL}
	\zbar^{(L)}(x,\mu,a^{(L)}):=
	\int\limits_{\R^{D_{L-1}}}\sigma^{(L-1)}\parn{\zbar^{(L-1)}(x,\mu),a^{(L-1)}}\,d\mu^{(L-1\mid L)}(a^{(L-1)}\mid a^{(L)}).
\end{equation}
This definition depends on the choice of regular conditional probability, but this issue will not concern us in what follows.

To finish, we define:
\begin{align}
\label{eq:defzbarL+1}
	&&\zbar^{(L+1)}(x,\mu)&:=
	\int\limits_{\R^{D_{L}}}\sigma^{(L)}\parn{\zbar^{(L)}(x,\mu,a^{(L)}),a^{(L)}}\,d\mu^{(L)}(a^{(L)})\\
	\mbox{ and }&& \ybar(x,\mu)&:=\sigma^{(L+1)}\parn{\zbar^{(L+1)}(x,\mu)}\nonumber.
\end{align}


\begin{remark}
\label{def:lbar}
Once we have the function $\ybar$, we can consider the mean-squared loss associated with a measure $\mu\in\Probspace(\R^D)$:
\[\Lbar(\mu) = \frac{1}{2}\Exp{(X,Y)\sim P}{|Y-\ybar(X,\mu)|^2}.\]
\end{remark}

\subsubsection{Mean-field versions of gradients.}
The next objects to be defined are the mean-field limits of the $M$ operators and the gradients presented in Section \ref{sub:backprop}. The idea here is that dependencies on $z^{(\ell)}_{i_\ell}$ are to be replaced by the corresponding $\zbar^{(\ell)}$.

Given $(x,\mu)\in \R^{d_X}\times \Probspace(\R^D)$, we first define

\begin{equation}
\label{eq:defMbarLplus1}
	\Mbar^{(L+1)}(x,\mu) := D\sigma^{(L+1)}\parn{\zbar^{(L+1)}(x,\mu)}.
\end{equation}

Then, we proceed as follows:
\begin{align}
\Mbar^{(L)}(x,\mu,a^{(L)}) &:= \Mbar^{(L+1)}(x,\mu) \cdot D_z\sigma^{(L)}\parn{\zbar^{(L)}(x,\mu,a^{(L)}), a^{(L)}},
\label{eq:defMbarL-Lminus1}\\
\Mbar^{(L-1)}(x,\mu) &:= {\displaystyle \int\limits_{\R^{D_{L}}}}\Mbar^{(L)}\parn{x,\mu,a^{(L)}}d\mu^{(L)}(a^{(L)})
\label{eq:defMbarLminus1}\\
 &\times{\displaystyle \int\limits_{\R^{D_{L-1}}}} D_z\sigma^{(L-1)}\parn{\zbar^{(L-1)}(x,\mu),a^{(L-1)}}\,d\mu^{(L-1,)}(a^{(L-1)})\nonumber.
\end{align}

Finally, we proceed recursively defining for $\ell\in [2:L-2]$:
\begin{equation}\label{eq:defMbarell}
\Mbar^{(\ell)}(x,\mu) =  \Mbar^{(\ell+1)}(x,\mu)\,\int\limits_{\R^{D_\ell}}\,D_z\sigma^{(\ell)}\parn{\zbar^{(\ell)}(x,\mu),a^{(\ell)}}\,d\mu^{(\ell)}(a^{(\ell)}).
\end{equation}

We may now define the mean-field equivalent of $\frac{d\yhat}{d\theta^{(\ell)}_{i_\ell,i_{\ell+1}}}$ that will dictate the evolution of the weights in the limit. For weights in the layer $\ell=1$, these gradients take the form
\[
	\gbar^{(1)}:\R^{D}\times \R^{d_X}\times \Probspace(\R^D)\to \R^{D_1},
\]
\begin{equation}
\label{eq:defgbar1}
	\gbar^{(1)}(\theta,x,\mu) = \Mbar^{(2)}(x,\mu)\,D_\theta\sigma^{(1)}\parn{\sigma^{(0)}(x,\theta^{(0)}),\theta^{(1)}}.
\end{equation}

For $\ell\in [2:L-2]$, we take
\[
	\gbar^{(\ell)}: \R^{D}\times \R^{d_X}\times \sM\to \R^{D_\ell},
\]
\begin{equation}
\label{eq:defgbarell}
	\gbar^{(\ell)}(\theta,x,\mu) := \Mbar^{(\ell+1)}(x,\mu)\,D_\theta\sigma^{(\ell)}\parn{\zbar^{(\ell)}(x,\mu),\theta^{(\ell)}}.
\end{equation}
Finally, for $\ell=L-1$ we take
\[
	\gbar^{(L-1)}:\R^{D}\times \R^{d_X}\times \sM\to \R^{D_{L-1}},
\]
\begin{equation}
\label{eq:defgbarL-1}
	\gbar^{(L-1)}(\theta,x,\mu) := \Mbar^{(L)}(x,\mu,\theta^{(L)})\,D_\theta\sigma^{(L-1)}\parn{\zbar^{(L-1)}(x,\mu),\theta^{(L-1)}}.
\end{equation}

We can define, analogously to \ref{eq:grad-ell}, a function as follows:
\begin{equation}
\label{def:Grad-ell}
\Grad^{(\ell)}(X,Y,\mu,\theta) =
\begin{cases}
\bold{0}_{\R^{D_\ell}} &\text{if } \ell\in\{0,L\},\\
\big(Y - \ybar(X,\mu)\big)^\dag\,\gbar^{(\ell)}(\theta,X,\soln_s)
& \ell\in[1:L-1].
\end{cases}
\end{equation}

Now that we have the mean-field version of the gradients, we can define the following McKean-Vlasov problem.

\begin{definition}[McKean-Vlasov problem for DNN]
\label{def:McKeanVlasov}
Let $\mu_0$ be a probability measure over $\R^{D}$. We say that a probability measure $\soln_{[0,T]}$ over $C([0,T],\R^D)$ is a solution to the McKean-Vlasov DNN problem with initial distribution $\mu_0$ if a random trajectory \[\Thetabar\sim \soln_{[0,T]}\] satisfies:
\begin{enumerate}
\item $\Thetabar(0)\sim \mu_0$;
\item for $\ell \in [0:L]$, $\Thetabar^{(\ell)}$ satisfies almost surely
\[
	\Thetabar^{(\ell)}(t) = \Thetabar^{(\ell)}(0) - \displaystyle{\int_0^t}\alpha(s)\,\Exp{(X,Y)\sim P}{\Grad^{(\ell)}(X,Y,\soln_s,\Thetabar_N(s))}ds,
\]
for all $t\in[0,T]$.
\end{enumerate}
\end{definition}

\begin{remark}[Vector notation]
\label{rem:vectorMcKeanVlasov}
With the above notation, define
\[
	\Grad(X,Y,\mu,\theta) = \parn{\Grad^{(\ell)}(X,Y,\mu,\theta),\ell\in[0:L]}\in \R^{D}.
\]
Then we may rewrite conditions in the above definition as saying that, if $\Thetabar\sim \soln_{[0,T]}$, then
\[
\begin{cases}
	\Thetabar(0)\sim \mu_0,\\
	\Thetabar(t) = \Thetabar(0) -
	\displaystyle{\int_0^t}\alpha(s)\cdot\Exp{(X,Y)\sim P}{\Grad(X,Y,\soln_t,\Thetabar(s))} ds &\mbox{a.s.}
\end{cases}
\]
\end{remark}

\begin{remark}
\label{rem:discontinuity}
The presence of a conditional distribution in the definition of $\zbar^{(L)}$ makes the drift term of Definition \ref{def:McKeanVlasov} potentially discontinuous as a function of the measure $\soln$, both in the weak and Wasserstein topologies. To the best of our knowledge, this kind of discontinuity has not been considered before in the literature on McKean-Vlasov problems. The proof of existence for the McKean-Vlasov problem for DNN will require that we identify a closed set $\Probspecial\subset \Probspace(C([0,T],\R^D))$ where $\zbar^{(L)}$ behaves well. This will be discussed in section \ref{sec:apriori_space}.\end{remark}


==> measureNN_aux/3-rigorous_results.tex <==
\subsection{Technical Assumptions.}\label{sub:assumptions}

In order to properly analyse our model, we start by delineating a series of assumptions. These are meant to be as broad as possible, while still allowing
the use of known analytical tools. We start by making a hypothesis on the initialization of the Network.

\begin{assumption}[Initialization]
\label{assump:initialization}
At time $t=0$, the weights
\[
	\theta^{(\ell)}_{i_\ell,i_{\ell+1}}(0)\in\R^{D_\ell}\,:\, 0\leq \ell\leq L,\;(i_\ell,i_{\ell+1}) \in [1:\boldN{\ell}{\ell+1}]
\]
are random and independent. Weights with the same superscript $\ell$ have a common law given by a probability measure $\mu^{(\ell)}_0\in \Probspace(\R^{D_\ell})$ with finite first moment.
\end{assumption}

Basically, this assumption means that initialization is independent and weights in the same layer share a common law. The next assumption deals with the nature of the activation functions.

\begin{assumption}[Activation functions are bounded with bounded derivatives]
\label{assump:activations} There exist a constant $C_{\ref{assump:activations}}>1$ with the following properties.

The data distribution $P$ of $(X,Y)\in\R^{d_X}\times \R^{d_Y}$ is such that $|Y|\leq C_{\ref{assump:activations}}$ almost surely. Moreover, the functions $\sigma^{(\ell)}$,  $\alpha$, and their Fr\'{e}chet derivatives are all bounded by $C_{\ref{assump:activations}}$ in the appropriate norms. In addition, each Fr\'{e}chet derivative of the $\sigma^{(\ell)}$ is also $C_{\ref{assump:activations}}$-Lipschitz. \ignore{More precisely, the following inequalities hold for all $\ell \in [0:L+1]$ and all $(z,\theta),(z',\theta')\in\R^{d_{\ell}}\times\R^{D_\ell}$:
\begin{enumerate}
\item $|\sigma^{(\ell)}(z,\theta)|\leq C_{\ref{assump:activations}}$ (where $|\cdot|$ is the Euclidean norm);
\item $\opnorm{D\sigma^{(\ell)}(z,\theta)}\leq C_{\ref{assump:activations}}$ (where $\pnorm{\text{Op}}{\cdot}$ is the operator norm);
\item $\opnorm{D\sigma^{(\ell)}(z,\theta) - D\sigma^{(\ell)}(z',\theta')} \leq C_{\ref{assump:activations}}\,(|z-z'| + |\theta - \theta'|)$.
\end{enumerate}
Finally, we assume that $D\sigma^{(L+1)}$ is bounded by $C_{\ref{assump:activations}}$ with with Lipschitz constant also bounded by $C_{\ref{assump:activations}}$ (we do {\em not} assume $\sigma^{(L+1)}$ itselt is bounded).}
\end{assumption}
Assumption \ref{assump:activations} is made for convenience, and excludes the popular ReLU nonlinearity. We expect that our results will extend with minor changes to more general activation functions.

\subsection{Main theorems.}

We now present our main results. The first one states that our McKean-Vlasov problem is well-posed.
\begin{theorem}[Existence and uniqueness of McKean-Vlasov solution; proof in Section \ref{sec:existence}]
\label{thm:independencestructure}
Under the assumptions in Section \ref{sub:assumptions}, the McKean-Vlasov problem in Section \ref{sub:McKeanVlasov} has a unique solution $\soln_{[0,T]}$. This solution has the following structure:
\begin{enumerate}
\item There exist deterministic functions \[\begin{array}{llllll}F^{(1)}&:&\R^{D_0}\times \R^{D_1}&\to& C([0,T],\R^{D_1});\\
F^{(\ell)}&:&\R^{D_\ell}&\to& C([0,T],\R^{D_\ell}), &\text{for } \ell\in [2:L-2]; \\
F^{(L-1)}&:&\R^{D_{L-1}}\times \R^{D_L}&\to&  C([0,T],\R^{D_{L-1}}),\end{array}\] such that, if $\Thetabar\sim \soln_{[0,T]}$, then almost surely, for all $t\in[0,T]$
\begin{align*}
	\Thetabar^{(1)}(t) =& F^{(1)}\parn{\Thetabar^{(0)}(0),\Thetabar^{(1)}(0)}(t),&\\
	\Thetabar^{(\ell)}(t) =& F^{(\ell)}\parn{\Thetabar^{(\ell)}(0)}(t),\quad\quad\quad\text{for }\ell\in [2:L-2],\\
	\Thetabar^{(L-1)}(t) =& F^{(L-1)}\parn{\Thetabar^{(L-1)}(0),\Thetabar^{(L)}(0)}(t).&
\end{align*}
\item As a consequence, $\soln_{[0,T]}$ factorizes into independent components, ie,
\[\soln_{[0,T]} = {\soln}^{(0,1)}_{[0,T]}\times\left(\prod_{\ell=2}^{L-2} {\soln}^{(\ell)}_{[0,T]} \right)\times {\soln}^{(L-1,L)}_{[0,T]}.\]
\end{enumerate}
\end{theorem}

Our second main results shows that we can describe the loss of our DNN with $N\gg 1$ particles in terms of the McKean-Vlasov limiting process.

\begin{theorem}[Approximation of errors; proof in Section \ref{sec:coupling}]\label{thm:error-approx}
Make the assumptions in the previous Section. Given $T>0$, let $\soln_{[0,T]}$ denote the unique solution of the McKean-Vlasov problem described in Subsection \ref{sub:McKeanVlasov}. Also, let $\left\{\btheta_N(k),\, k\in \left[0:\left\lceil\frac{T}{\eps}\right\rceil\right]\right\}$ be steps in the SGD process for the DNN described in Subsection \ref{sub:DNN_definition}.

Then, for all $k\in \left[0:\left\lceil\frac{T}{\eps}\right\rceil\right]$, it holds that:
\begin{equation}
\label{eq:error-general}
\Exp{\stackrel{(X_k,Y_k) \stackrel{\tiny{iid}}{\sim} P}{\btheta_N(0)\sim \mu_0}}{\abs{L_N(\btheta_N(k)) - \Lbar(\soln_{k\eps})}}\leq C_{\ref{thm:error-approx}}\,\left(\frac{1}{\sqrt{N}}+\eps\right)
\end{equation}
where $C_{\ref{thm:error-approx}}$ depends only on $C_{\ref{assump:activations}}$, the inner dimensions $\{d_\ell,\, \ell\in[0:L+1]\}$ and the number of hidden layers $L$.
\end{theorem}

In fact, our proofs also give a "microscopic" approximation of SGD, whereby we approximate individual weights of the network. 
\begin{theorem}[Approximation by ideal particles; proof in Section \ref{sec:coupling}]\label{thm:microscopic} Under the assumptions in Section \ref{sub:assumptions}, consider $\soln_{[0,T]}$ as in Theorem \ref{thm:independencestructure}, and let \[\left\{\btheta_N(k),\, k\in \left[0:\left\lceil\frac{T}{\eps}\right\rceil\right]\right\}\]
be as in Theorem \ref{thm:error-approx}. Then one can couple the above evolution with certain "ideal particles"
\[\left\{\bthetabar_N(t)\in\R^{p_N},\, t\in [0,T]\right\}\]
so that:
\begin{enumerate}
\item the trajectories $\thetabar^{(\ell)}_{i_\ell,i_{\ell+1},[0,T]}$ for $\ell\in [0:L]\backslash\{1,L-1\}$ and $(i_\ell,i_{\ell+1})\in [1:N_\ell]\times [1:N_{\ell+1}]$ are all independent, and each $\thetabar^{(\ell)}_{i_\ell,i_{\ell+1},[0,T]}\sim {\soln}^{(\ell)}_{[0,T]}$;
\item conditionally on the above, $\thetabar^{(\ell)}_{i_\ell,i_{\ell+1},[0,T]}$ for $\ell\in \{1,L-1\}$ and $(i_\ell,i_{\ell+1})\in [1:N_\ell]\times [1:N_{\ell+1}]$ are independent, with each \[\thetabar^{(1)}_{i_1,i_{2},[0,T]}\sim {\soln}_{[0,T]}^{(1\mid 0)}(\cdot\mid  \thetabar^{(0)}_{1,i_{1},[0,T]})\] and each \[\thetabar^{(L-1)}_{i_{L-1},i_{L},[0,T]}\sim {\soln}^{(L-1\mid L)}_{[0,T]}(\cdot\mid  \thetabar^{(L)}_{i_L,1,[0,T]});\]
\item finally, for each choice of input-to-output path $i_0,i_1,\dots,i_L,i_{L+1}$ with $i_{0}=i_{L+1}=0$ and $i_\ell\in [1:N_\ell]$ for $\ell\in [1:L]$, we have:
\[(\thetabar^{(0)}_{i_\ell,i_{\ell+1},[0,T]}\,:\, \ell\in [0:L])\sim \soln_{[0,T]},\]
and for all $k\in [0: \lceil T/\eps\rceil ]$:
\[\Exp{\stackrel{(X_k,Y_k) \stackrel{\tiny{iid}}{\sim} P}{\btheta_N(0)\sim \mu_0}}{\sum_{\ell=0}^L|\theta^{(\ell)}_{i_\ell,i_{\ell+1}}(k) - \thetabar^{(\ell)}_{i_\ell,i_{\ell+1}}(k\eps)|}\leq C_{\ref{thm:microscopic}}\,\left(\frac{1}{\sqrt{N}}+\eps\right).\]
\end{enumerate}\end{theorem}

\begin{remark}[Propagation of chaos: weights versus paths]\label{rem:propagationofchaos} One key difference between our system and and other interacting particle systems of mean-field type (eg. as popularized by \cite{Sznitman1991}) is that network weights do {\em not} become independent in the limit, as even ideal particles have nontrivial dependencies. However, disjoint {\em paths of weights} will become independent. This implies a propagation of chaos for most finite sets of paths. This is in keeping with the point made in Section \ref{sec:setup} where we noted that paths are the fundamental units of our system.\end{remark}

\subsection{Comparison with related results} \label{sub:comparison} As noted, there are two recent preprints that tackle similar problems to our main results. Nguyen \cite{Nguyen2019} has essentially the same ansatz and the same end result as we do, but he uses nonrigorous methods. 

By contrast, Sirignano and Spiliopoulos \cite{Sirignano2019} consider networks with $L\geq 3$ and $N_\ell$ units in each layer, but then make the $N_\ell$ diverge one at a time. As they observe in \cite[\S 2.2]{Sirignano2019}, to consider all $N_\ell$ diverging simultaneously, one alternative would be to write an empirical measure for the weights, and then write the dynamics of SGD as a closed dynamics over empirical measures. This would be the natural extension of work on the shallow case \cite{MeiArxiv2018,Rotskoff2018,Sirignano2018}. However, Sirignano and Spiliopoulos note that there are difficulties with this and related ideas. 

Our own work seems to identify one important source of the above difficulties. The most natural measure to consider is over paths of weights. Then, however the closed evolution obtained turns out to involve conditional measures, and conditioning is a discontinuous operation. In our approach, we have {\em not} tried to write a single empirical measure for all weights. Rather, our approach follows the ideas outlined in the next section. 

==> measureNN_aux/A2-apriori_space.tex <==
In this section we continue the work of Section \ref{sec:apriori_simple}. Corollary \ref{cor:mappingwelldefined} shows that there is a well-defined map $\psi$ whose fixed points are solutions of the McKean Vlasov problem. It is then natural to iterate that map to obtain existence and uniqueness of solutions.

To make this work, we will need some analytic properties of the functions $G_{\nu}^{(\ell)}$ appearing in Lemma \ref{lem:constrainstructure}. For $\ell\neq L-1$ one could show  that these functions are Lipschitz, which is enough for our purposes. However, the function $G_{\nu}^{(L-1)}$ is a bit more delicate because, in principle, it could be that the dependence on $\Thetabar^{(L)}(0)$ is not "nice". This is related to Remark \ref{rem:discontinuity}.

To circumvent such problems, we will show that we can further constrain the set of potential solutions of our problem. We will define the set of $R$-special measures (Definition \ref{def:Rspecialmeasure}) so that a mesure $\nu_{[0,T]}$ in this set will have special Lipschitz properties in its $(L-1)^\text{th}$ coordinate. The results in this section will imply that this set is well-behaved with respect to $\psi$ and that the search for solutions can be narrowed down to this set.

To make all of this precise, we need two new definitions. The first defines the property we want the $(L-1)^\text{th}$ coordinate process to obey.

\begin{definition}[$R$-special function]\label{def:Rspecialfunction}Given $R>0$, we say that \[F:\R^{D_{L-1}}\times \R^{D_L}\to C([0,T],\R^{D_{L-1}})\] is {\em $R$-special} if:
\begin{enumerate}
\item For any $a=(a^{(L-1)},a^{(L)})\in \R^{D_{L-1}}\times \R^{D_L}$, the trajectory
\[t\in [0,T]\mapsto F(a)(t)\in \R^{D_{L-1}}\]
is $R$-Lipschitz in $t$, and $F(a)(0)=a^{(L-1)}$.
\item For any $t\in [0,T]$, the mapping
\[a=(a^{(L-1)},a^{(L)})\in \R^{D_{L-1}}\times \R^{D_L}\mapsto F(a)(t)\in \R^{D_{L-1}}\]
is $e^{Rt}$-Lipschitz as a function of $a$.\end{enumerate}
\end{definition}

The second definition defines the set of probability measures we will work with.

\begin{definition}[$R$-special measure]\label{def:Rspecialmeasure} A measure \[\mu_{[0,T]}\in \Probspace(C([0,T],\R^D))\] is said to be $R$-special if $\mu_{[0,T]}\in \Probspace_R$ and there exists an $R$-special function $F_\mu$ such that, if $\Theta\sim \mu_{[0,T]}$, for all $t\in[0,T]$
\[\Theta^{(L-1)}(t) = F_\mu\parn{\Theta^{(L-1)}(0),\Theta^{(L)}(0)}(t)\mbox{ almost surely.}\]
The set of all $R$-special measures is denoted by $\Probspecial_R$.\end{definition}

To finish this section, we will show that the discontinuity issues raised in Remark \ref{rem:discontinuity} disappears when we restrict to $R$-special measures. Moreover, they allow us to estimate the difference between the values of $\zbar^{(L)}$ for different measures. We will do that by stating several Lemmas, whose proofs will be carried out in the next subsections.

\begin{lemma}[Proof in \S \ref{sub:proofredefiningzL}]
\label{lem:redefiningzL}
When $\nu_{[0,T]}\in \Probspecial_R$, we have that, for $\mu_0^{(L)}$-almost every $a^{(L)}\in \R^{D_L}$ and $t\in [0,T]$:
\[
\zbar^{(L)}(x,\nu_t,a^{(L)}) =\int\limits_{\R^{D_{L-1}}}\fsigma{L-1}{\zbar^{(L-1)}(x,\nu_t),F_\nu\parn{\tilde{a}^{(L-1)},a^{(L)}}(t)}\,d\mu_0^{(L-1)}\parn{\tilde{a}^{(L-1)}}.
\]
\end{lemma}

\begin{lemma}[Proof in \S \ref{sub:proofestimatezbarL}]\label{lem:estimatezbarL}When $\tilde{\nu}_{[0,T]},\nu_{[0,T]}\in \Probspecial_R$, we have that, for all $t\in [0,T]$ and $x\in\R^{d_X}$:
\[\int\limits_{\R^{D_L}}\abs{\zbar^{(L)}(x,\tilde{\nu}_t,a^{(L)}) - \zbar^{(L)}(x,\nu_t,a^{(L)})}\,d\mu^{(L)}_0\parn{a^{(L)}}\leq C_{\ref{assump:activations}}\cdot(e^{Rt}+1)\,W(\tilde{\nu}_{[0,t]},\nu_{[0,t]}).\]\end{lemma}

The next two Lemmas  are the main results about $R$-special measures. Lemma \ref{lem:specialclosedpsi} shows that this set is closed under the mapping $\psi$ while Lemma \ref{lem:specialcontainssoln} that all solutions must be $R$-special.

\begin{lemma}[Special measures are closed under $\psi$; Proof in \S \ref{sub:proofpsispecial}]
\label{lem:specialclosedpsi} There exists a value $R_{\ref{lem:specialclosedpsi}}>0$ depending only on $C_{\ref{assump:activations}}$ and $L$ such that, for all $R\geq R_{\ref{lem:specialclosedpsi}}$, the mapping $\psi$ introduced in Corollary \ref{cor:mappingwelldefined} satisfies $\psi(\Probspecial_R)\subset \Probspecial_R$.
\end{lemma}

\begin{lemma}[All solutions are special; Proof in \S \ref{sub:proofspecialcontainssoln}]
\label{lem:specialcontainssoln}
There exists a value $R_{\ref{lem:specialcontainssoln}}$ depending only on $C_{\ref{assump:activations}}$ and $L$ such that, for all $R\geq R_{\ref{lem:specialcontainssoln}}$, any solution to the McKean-Vlasov problem belongs to $\Probspecial_{R}$.
\end{lemma}

Finally, we mention an important technical result, to be proved in Appendix \ref{sec:Probspecialisclosed}.

\begin{theorem}[Special measures form a closed set]
\label{thm:Probspecialisclosed}
The set $\Probspecial_R$ is closed under weak convergence (and thus also under Wasserstein $L^1$ metric).
\end{theorem}

Now we proceed onto the proofs of the above Lemmas.

\subsection{Proof of a formula for $\zbar^{(L)}$ with a $R$-special measure}
\label{sub:proofredefiningzL}
\begin{proof}[Proof of Lemma \ref{lem:redefiningzL}]
Let $\Theta \sim \nu_{[0,T]}\in\Probspecial_R$. Then $\Theta^{(L)}$ is a.s. constant and
\[\Pr{\forall t\in [0,T]\,:\,
	\Theta^{(L-1)}(t) = F_\nu\parn{\Theta^{(L-1)}(0),\Theta^{(L)}(0)}(t)}=1.
\]
We also have
\[
	(\Theta^{(L-1)}(0),\Theta^{(L)}(0)) = (\Theta^{(L-1)}(0),\Theta^{(L)}(t))\sim \mu_0^{(L-1,L)} = \mu_0^{(L-1)}\times \mu_0^{(L)}.
\]
Therefore,
\[
	\mu_t^{(L-1\mid L)}(\cdot\mid a^{(L)}) =
	\int\limits_{\R^{D_{L-1}}}\,{\boldsymbol \delta}_{F_\nu(a^{(L-1)},a^{(L)})(t)}\,d\mu_0^{(L-1)}(a^{(L-1)})\mbox{ for all $t\in[0,T]$, a.s., }
\]
where ${\boldsymbol \delta_\cdot}$ is a Dirac delta. Plugging this into Equation \eqnref{defzbarL} which defines $\zbar^{(L)}$ finishes the proof.
\end{proof}

\subsection{Differences of $\zbar^{(L)}$ for $R$-special measures}
\label{sub:proofestimatezbarL}
We now show how to estimate differences in $\zbar^{(L)}$ for $R$-special measures.
\begin{proof}[Proof of Lemma \ref{lem:estimatezbarL}]
Recall from Lemma \ref{lem:redefiningzL} that:
\[\zbar^{(L)}(x,\nu_t,a^{(L)}) =\int\limits_{\R^{D_{L-1}}}\fsigma{L-1}{\zbar^{(L-1)}(x,\mu),F_\nu\parn{\tilde{a}^{(L-1)},a^{(L)}}(t)}\,d\mu_0^{(L-1)}(\tilde{a}^{(L-1)})\]
and similarly for $\zbar^{(L)}(x,\tilde{\nu}_t,a^{(L)})$. Since $\sigma^{(L-1)}$ is $C_{\ref{assump:activations}}$-Lipschitz, then
\begin{align*}
&\abs{\zbar^{(L)}(x,\nu_t,a^{(L)}) - \zbar^{(L)}(x,\tilde{\nu}_t,a^{(L)})} \leq \\
&\quad\quad\quad C_{\ref{assump:activations}}\cdot\int\limits_{R^{D_{L-1}}}\abs{F_\nu\parn{\tilde{a}^{(L-1)},a^{(L)}}(t) - F_{\tilde{\nu}}\parn{\tilde{a}^{(L-1)},a^{(L)}}(t)}\,d\mu^{(L-1)}_0(\tilde{a}^{(L-1)}).
\end{align*}
It follows that, in order to prove the Lemma, it suffices to show that:
\begin{equation}
\label{eq:goalestimatezbarL}
\mbox{\bf Goal: } \int\limits_{\R^{D_{L-1}}\times \R^{D_{L}}}|F_\nu(a)(t) - F_{\tilde{\nu}}(a)(t))|\,d\mu^{(L-1,L)}_0(a)\leq (e^{Rt}+1)\cdot W(\nu_{[0,t]},\tilde{\nu}_{[0,t]}),
\end{equation}
where as usual we write $a=(a^{(L-1)},a^{(L)})\in\R^{D_{L-1}}\times \R^{D_L}$.

To achieve this goal, let $\Theta\sim \nu_{[0,t]}$, $\tilde{\Theta}\sim \tilde{\nu}_{[0,t]}$ be a coupling of $ \nu_{[0,t]}$ and $\tilde{\nu}_{[0,t]}$ that achieves Wasserstein distance:
\[
\Ex{\sup_{0\leq r\leq t}|\Theta(r) - \tilde{\Theta}(r)|}=W(\nu_{[0,t]},\tilde{\nu}_{[0,t]}).
\]
The quantity in the LHS of (\ref{eq:goalestimatezbarL}) may be rewritten as:
\[
(I):=\Ex{\abs{F_\nu\parn{\Theta^{(L-1)}(0),\Theta^{(L)}(0)}(t) - F_{\tilde{\nu}}\parn{\Theta^{(L-1)}(0),\Theta^{(L)}(0)}(t)}}.
\]
Moreover, because the two measures are special, we have the almost-sure identities:
\begin{align*}
F_\nu\parn{\Theta^{(L-1)}(0),\Theta^{(L)}(0)}(t) =& \Theta^{(L-1)}(t);\\
F_{\tilde{\nu}}\parn{\tilde{\Theta}^{(L-1)}(0),\tilde{\Theta}^{(L)}(0)}(t) =& \tilde{\Theta}^{(L-1)}(t).
\end{align*}
We also know that $F_{\tilde{\nu}}$ is an $R$-special function, which implies that $F_{\tilde{\nu}}(\cdot)(t)$ is $e^{Rt}$-Lipschitz (as per Definition \ref{def:Rspecialfunction}). In particular, we have that:
\[
\abs{F_{\tilde{\nu}}\parn{\tilde{\Theta}^{(L-1)}(0),\tilde{\Theta}^{(L)}(0)}(t) - F_{\tilde{\nu}}\parn{\Theta^{(L-1)}(0),\Theta^{(L)}(0)}(t)}\leq e^{Rt}\cdot\abs{\Theta(0) - \tilde{\Theta}(0)}.
\]
We conclude that:
\begin{align*}
(I) \leq & \Ex{\abs{F_\nu\parn{\Theta^{(L-1)}(0),\Theta^{(L)}(0)}(t)-F_{\tilde{\nu}}\parn{\tilde{\Theta}^{(L-1)}(0),\tilde{\Theta}^{(L)}(0)}(t)}} \\
   &\quad +  \Ex{\abs{F_{\tilde{\nu}}\parn{\Theta^{(L-1)}(0),\Theta^{(L)}(0)}(t)-F_{\tilde{\nu}}\parn{\tilde{\Theta}^{(L-1)}(0),\tilde{\Theta}^{(L)}(0)}(t)}}\\
  \leq & \Ex{\abs{\Theta^{(L-1)}(t)-\tilde{\Theta}^{(L-1)}(t)}} + e^{Rt}\cdot\Ex{\abs{\Theta(0) - \tilde{\Theta}(0)}}\\
  \leq & (e^{Rt}+1)\cdot\Ex{\sup_{0\leq r\leq t}\abs{\Theta(r) - \tilde{\Theta}(r)}}= (e^{Rt}+1)\cdot W(\nu_{[0,t]},\tilde{\nu}_{[0,t]}),
\end{align*}
which achieves Goal \eqref{eq:goalestimatezbarL}.
\end{proof}


\subsection{Proof that special measures are closed under $\psi$.}\label{sub:proofpsispecial}
Now we move on to prove Lemma \ref{lem:specialclosedpsi}, which shows that the map $\psi$ maps $\Probspecial_R$ onto itself, assuming $R$ is large enough.

\begin{proof}[Proof of Lemma \ref{lem:specialclosedpsi}] Let $\nu_{[0,T]}\in\Probspecial_{R}$ for some $R$ to be specified later. Lemma \ref{lem:constrainstructure} indicates that there exists a function $G_{\nu}^{(L-1)}:\R^{D_{L-1}}\times \R^{D_L}\to C([0,T],\R^{D_{L-1}})$ such that, if $\Thetabar\sim \psi(\nu_{[0,T]})$, then almost surely $\Thetabar^{(L-1)}(t)=G_{\nu}^{(L-1)}\parn{\Thetabar^{(L-1)}(0),\Thetabar^{(L)}(0)}(t)$ for all $t\in[0,T]$. Our goal is to show that:
\begin{equation}
\label{eq:goalspecialclosedpsi}
\mbox{{\bf Goal:} } G_{\nu}^{(L-1)}(\cdot)= G(\cdot)\qquad\mbox{ $\mu_0^{(L-1,L)}$-a.e., for some $R$-special function $G$,}
\end{equation}
which clearly suffices to prove the Lemma.

To do this, we investigate  the ODE \ref{eq:ODETheta-L} satisfied by $\Thetabar^{(L-1)}$ under the assumption that $\nu_{[0,T]}$ is $R$-special. We will need the following result, which is a direct consequence of Picard iteration.

\begin{proposition}[Proof in \S  \ref{sub:proofPicardsimple}]
\label{prop:Picardsimple}
Fix constants $R\geq 2V_{\ref{prop:Picardsimple}} > 0$.
Given $(a^{(L-1)},a^{(L)})$ consider the initial value problem
\begin{equation}
\label{eq:H-ODE}
\left\{\begin{array}{rll}
x(0) =&a^{(L-1)}\\
\dfrac{dx}{dt}(t) =& H\parn{t,x(t),a^{(L)}} & \text{for }t\in [0,T],
\end{array}\right.
\end{equation}
where $H:[0,T]\times \R^{D_{L-1}}\times \R^{D_{L}}\to \R^{D_{L-1}}$ is a continuous map satisfying the following properties:
\begin{enumerate}
\item $H$ is uniformly bounded by $V_{\ref{prop:Picardsimple}}$;
\item for each fixed $t\in [0,T]$ and $a^{(L-1)}\in \R^{D_{L-1}}$, the map
\[a^{(L)}\in \R^{D_{L}}\mapsto H(t,a^{(L-1)},a^{(L)})\] is $V_{\ref{prop:Picardsimple}}\cdot e^{Rt}$-Lipschitz;
\item for each fixed $t\in [0,T]$ and $a^{(L)}\in \R^{D_{L}}$,
\[a^{(L-1)}\in \R^{D_{L}}\mapsto H(t,a^{(L-1)},a^{(L)})\] is $V_{\ref{prop:Picardsimple}}$-Lipschitz.
\end{enumerate}
Then the map
\[G:\R^{D_{L-1}}\times \R^{D_{L}}\to C([0,T],\R^{D_{L-1}})\]
that associates to each $(a^{(L-1)},a^{(L)})$, the solution of \ref{eq:H-ODE} is an $R$-Special function.
\end{proposition}

Given this Proposition, Lemma \ref{lem:specialclosedpsi} follows from the following result.

\begin{claim}
\label{claim:Hexists}
Let $\nu_{[0,T]}\in\Probspecial_R$. Then there exists a constant $V_{\ref{claim:Hexists}}=V_{\ref{claim:Hexists}}(C_{\ref{assump:activations}},L)$ and a continuous function
\[
H:[0,T]\times \R^{D_{L-1}}\times \R^{D_{L}}\to \R^{D_{L-1}}\mbox{ (possibly depending on $\nu_{[0,T]}$)}
\]
satisfying properties (1) - (3) in the proposition above with $V_{\ref{prop:Picardsimple}} = V_{\ref{claim:Hexists}}$, and so that, if $\Thetabar\sim \psi(\nu_{[0,T]})$, then almost surely, for all $t\in[0,T]$
\begin{equation}
\Thetabar^{(L-1)}(t) = \Thetabar^{(L-1)}(0) + \int_0^{t}\,H\parn{s,\Thetabar^{(L-1)}(s),\Thetabar^{(L)}(0)}\,ds.
\end{equation}
\end{claim}
Indeed, we may apply Proposition \ref{prop:Picardsimple} to the $H$ coming from this Claim to deduce that, if $R\geq R_{\ref{lem:specialclosedpsi}}(C_{\ref{assump:activations}},L):=2V_{\ref{claim:Hexists}}(C_{\ref{assump:activations}},L)$ and $\nu_{[0,T]}\in\Probspecial_R$, then for $\Thetabar\sim\psi(\nu_{[0,T]})$ and for all $t\in[0,T]$
\[
\Thetabar^{(L-1)}(t)=G_\nu^{(L-1)}\parn{\Thetabar^{(L-1)}(0),\Thetabar^{(L)}(0)}(t) =  G\parn{\Thetabar^{(L-1)}(0),\Thetabar^{(L)}(0)}(t) \mbox{ a.s.,}
\]
where $G$ is the $R$-special function from Proposition \ref{prop:Picardsimple}. In particular, this implies Goal (\ref{eq:goalspecialclosedpsi}).

We now prove the Claim. In what follows, we will use symbols $V_0,V_1,\dots$ to denote positive quantities that depend only on $C_{\ref{assump:activations}}$ and $L$.

Consider $\nu_{[0,T]}\in \Probspecial_R$. From Lemma \ref{lem:constrainstructure} we know that there exists an $R$-special function $F_\nu$ such that the identity
\begin{equation}
\label{eq:zbarLredefined}
\zbar^{(L)}(x,\mu_t,a^{(L)}) =\int\limits_{\R^{D_{L-1}}}\fsigma{L-1}{\zbar^{(L-1)}(x,\mu),F_\nu\parn{\tilde{a}^{(L-1)},a^{(L)}}(t)}\,d\mu_0^{(L-1)}(\tilde{a}^{(L-1)})
\end{equation}
holds simultaneously for all $t\in [0,T]$, $P$-a.e $x\in\R^{d_X}$ for $\mu_0^{(L)}$-a.e. $a^{(L)}\in\R^{D_L}$.

In a slight abuse of notation, we will assume that $\zbar^{(L)}$ has been redefined so that (\ref{eq:zbarLredefined}) holds for {\em all} $a^{(L)}\in \R^{D_{L}}$ and $x\in \R^{d_X}$. Recalling that $\sigma^{(L-1)}$ is $C_{\ref{assump:activations}}$-Lipschitz and $F_\nu(\cdot)(t)$ is $e^{Rt}$-Lipschitz (because $F_\nu$ is $R$-special), we easily obtain that:
\begin{equation}
\label{eq:zbarLLipschitz}
\forall t\in[0,T]\,:\,\zbar^{(L)}(x,\nu_t,a^{(L)}) \mbox{ is a $C_{\ref{assump:activations}}\cdot e^{Rt}$-Lipschitz function of $a^{(L)}$}.
\end{equation}
Now consider the drift term for the $(L-1)^\text{th}$ particle. Recalling Assumption \ref{assump:activations}, Lemma \ref{lem:redefiningzL}, and the definitions in \ref{sub:McKeanVlasov} we see that
\[\Mbar^{(L)}(x,\nu_t,a^{(L)}) = \Mbar^{(L+1)}(x,\nu_t)\,D_z\fsigma{L}{\zbar^{(L)}(x,\nu_t,a^{(L)})}\]
is continuous in $(t,a^{(L)})$, $V_0\cdot e^{Rt}$-Lipschitz in $a^{(L)}$ for $t\geq 0$ fixed, and bounded by $V_0$. Also, for ${\bf a}=(a^{(\ell)})_{\ell=0}^{(L)}\in \R^D$
\[
\gbar^{(L-1)}(x,\nu_t,{\bf a}) = \Mbar^{(L)}(x,\nu_t,a^{(L)})\,D_\theta\fsigma{L-1}{\zbar^{(L)}(x,\nu_t,a^{(L)}),a^{(L-1)}}
\]
is continuous in $(t,a^{(L-1)},a^{(L)})$, $C_{\ref{assump:activations}}$-Lipschitz in $a^{(L-1)}$ and $V_1\cdot e^{Rt}$-Lipschitz in $a^{(L)}$ for $t\geq 0$ fixed. $\gbar^{(L-1)}$ is also uniformly bounded by $V_1$. Once we notice additionally that $\gbar^{(L-1)}(x,\nu_t,{\bf a})$ depends on ${\bf a}$ only through $a=(a^{(L-1)},a^{(L)})$, we may define
\[H(t,a) = H(t,a^{(L-1)},a^{(L)}):= -\alpha(t)\,\Ex{(Y-\ybar(X,\nu_t))^\dag\,\gbar^{(L-1)}(x,\nu_t,{\bf a})},\]
for $(t,a)\in [0,T]\times \R^{D_{\ell-1}}\times \R^{D_\ell}$ (with ${\bf a} = (a^{(\ell)})_{\ell=0}^L$ arbitrarily defined for $\ell\neq L,L-1$). Clearly,  $H$ has the desired properties, as per Assumption \ref{assump:activations} and the previous bounds.
\end{proof}

\subsection{Proof that all solutions are special.}
\label{sub:proofspecialcontainssoln}
We now argue that all fixed points $\soln$ of $\psi$ are $R$-special.
\begin{proof}[Proof of Lemma \ref{lem:specialcontainssoln}]
The proof of this result is similar to that of Lemma \ref{lem:specialclosedpsi} in Section \ref{sub:proofpsispecial}. The key difference is that we will analyse a slightly more complicated Cauchy problem than the one in Proposition \ref{prop:Picardsimple}.

Let $\soln_{[0,T]}\in \Probspace(C([0,T],\R^D))$ be a solution to the McKean-Vlasov Problem in Definition \ref{def:McKeanVlasov}. Lemma \ref{lem:trivialsoln} implies that $\soln_{[0,T]}\in\Probspace_R$ if $R\geq R_{\ref{lem:trivialsoln}}$. Corollary \ref{cor:mappingwelldefined} applies to $\soln_{[0,T]}$, and we have $\psi(\soln_{[0,T]})=\soln_{[0,T]}$ because $\soln_{[0,T]}$ is a solution. Lemma \ref{lem:constrainstructure} implies there exist a measurable mapping $\Gsoln:=G_{\soln}^{(L-1)}$ such that if $\Thetabar\sim \soln_{[0,T]}$, then
\begin{equation}
\label{eq:Gisusefulforsoln}
\Thetabar^{(L-1)}(t) = \Gsoln\parn{\Thetabar^{(L-1)}(0),\Thetabar^{(L)}(0)}(t) \quad\forall t\in[0,T] \mbox{ a.s..}
\end{equation}

We also know from Lemma \ref{lem:constrainstructure} that $\Gsoln$ belongs to the following set of functions if $R\geq  R_{\ref{lem:trivialsoln}}$
\begin{equation}
\label{eq:defsU}
\sU:=\left\{g:\R^{D_{L-1}}\times \R^{D_L} \to C([0,T],\R)\,:\,
\begin{array}{l}
\mbox{$g$ is measurable;}\\
t\mapsto g(a)(t) \mbox{ is $R$-Lipschitz}\\
\forall a\in \R^{D_{L-1}}\times \R^{D_L};\\
g(a)(0)=a^{(L-1)}
\end{array}\right\}.
\end{equation}

Our goal will be to show:
\begin{equation}
\label{eq:goalspecialcontainssoln}
\mbox{{\bf Goal:} $\Gsoln$ is a.s. equal to an $R$-special function $G_o$, if $R\geq R_1(C,L)$.}
\end{equation}
Indeed, this will imply that $\soln_{[0,T]}$ is $R$-special, as per Definition \ref{def:Rspecialmeasure}.

To do this, we will need to "do analysis" on the set $\sU$. We need to establish some additional notation. For $g_1,g_2\in\sU$ and $t\in [0,T]$, we define.
\begin{equation}
\label{eq:distU}
\dist(g_1,g_2;t):=\sup\limits_{a\in \R^{D_{L-1}}\times \R^{D_L}}\abs{g_1(a)(t) - g_2(a)(t)}
\end{equation}
and note that $\dist(g_1,g_2;t)\leq 2Rt$ because each $g_i$ is $R$-Lipschitz and $g_1(a)(0)=g_2(a)(0)=a^{(L-1)}$ for each $a\in \R^{D_{L-1}}\times \R^{D_L}$.

The next Proposition gives properties of a nonstandard Cauchy-type problem for functions in $\sU$. It should be contrasted with Proposition \ref{prop:Picardsimple} in the proof of Lemma \ref{lem:specialclosedpsi}.

\begin{proposition}[Proof in Appendix \ref{sub:proofPicardcomplicated}]
\label{prop:Picardcomplicated}
Fix $R\geq 2V_{\ref{prop:Picardcomplicated}}>0$ constants and let
\[
\Xi:[0,T]\times \R^{D_{L-1}}\times \R^{D_L}\times \sU\to \R^{D_{L-1}}
\]
be a measurable function that satisfies the following properties:
\begin{enumerate}
\item $\Xi$ is uniformly bounded by $V_{\ref{prop:Picardcomplicated}}$.
\item If two functions $g_1,g_2\in\sU$ are such that $g_1(a^{(L-1)},a^{(L)})=g_2(a^{(L-1)},a^{(L)})$ $\mu_0^{(L-1)}\times \mu_0^{(L)}$-almost surely, then:
\[
\Xi\parn{t,a^{(L-1)},a^{(L)},g_1}=\Xi\parn{t,a^{(L-1)},a^{(L)},g_2}
\]
$\mu_0^{(L-1)}\times \mu_0^{(L)}$-almost-surely;
\item for any fixed $g\in \sU$, the map
\[
(t,a^{(L-1)},a^{(L)})\mapsto \Xi\parn{t,a^{(L-1)},a^{(L)},g}
\]
is measurable. Also, for $a^{(L)}$ fixed, then $(t,a^{(L-1)})\mapsto \Xi\parn{t,a^{(L-1)},a^{(L)},g}$ is continuous;
\item for any fixed $t\in [0,T]$, $g\in \sU$ and $a,b\in \R^{D_{L-1}}\times \R^{D_L}$ with $|a-b|\leq \epsilon$
\begin{align*}
&\abs{\Xi\parn{t,a^{(L-1)},a^{(L)},g} - \Xi\parn{t,b^{(L-1)},b^{(L)},g}}\\
&\qquad\qquad\qquad\leq V_{\ref{prop:Picardcomplicated}}\,\sup\limits_{\stackrel{a',b'\in\R^{D_{L-1}}\times \R^{D_L}}{|a'-b'|\leq \epsilon}}\abs{g(a')(t)-g(b')(t)};
\end{align*}
\item for any fixed $t\in [0,T]$, $g_1,g_2\in \sU$ and $a\in \R^{D_{L-1}}\times \R^{D_L}$:
\[
\abs{\Xi(t,a^{(L-1)},a^{(L)},g_1) - \Xi(t,a^{(L-1)},a^{(L)},g_2)}\leq V_{\ref{prop:Picardcomplicated}}\cdot\dist(g_1,g_2;t).
\]
\end{enumerate}
Then there exists a mapping
\[\sT:\sU\to \sU\]
such that, for $g\in \sU$, $a = (a^{(L-1)},a^{(L)})\in \R^{D_{L-1}}\times \R^{D_L}$, and $t\in[0,T]$,
\begin{equation}
\label{eq:defTsoln}
\sT(g)(a)(t) = a^{(L-1)} + \int_0^t\,\Xi\parn{s,g(a)(t),a^{(L)},g}\,ds.
\end{equation}
Moreover, $\sT$ has an unique fixed point $G_o$ which is an $R$-special function. If $\tilde{G}\in\sU$ satisfies $\sT(\tilde{G})=\tilde{G}$ $\mu_0^{(L-1)}\times \mu_0^{(L)}$-a.e., then $\tilde{G}=G_o$ $\mu_0^{(L-1)}\times \mu_0^{(L)}$-a.e..
\end{proposition}

We now make the following Claim.

\begin{claim}[Proven below]
\label{claim:Xiexists}
There exist a constant $V_{\ref{claim:Xiexists}} = V_{\ref{claim:Xiexists}}(C_{\ref{assump:activations}},L)>0$ and a function:
\[
\Xi:[0,T]\times \R^{D_{L-1}}\times \R^{D_L}\times \sU\to \R^{D_{L-1}}
\]
satisfying assumptions (1) - (5) in Proposition \ref{prop:Picardcomplicated}, and so that, for $\mu_0$-a.e initial condition and for all $t\in [0,T]$:
\[
\Thetabar^{(L-1)} (t) = \Thetabar^{(L-1)}(0) + \int_0^t\,\Xi\parn{s,\Thetabar^{(L-1)}(t),\Thetabar^{(L)}(0),\Gsoln}\,ds.
\]
\end{claim}

Once we prove this claim, the theorem is essentially proved. We just need to apply Proposition \ref{prop:Picardcomplicated} with this function $\Xi$ together with Lemma \ref{lem:constrainstructure}. The upshot is that, if $R\geq R_{\ref{lem:specialcontainssoln}}:=2V_{\ref{claim:Xiexists}}$, then the following identity holds almost surely, simultaneously for all $t\in [0,T]$:
\begin{align*}
&\Gsoln(\Thetabar^{(L-1)}(0),\Thetabar^{(L)}(0))(t) =\, \Thetabar^{(L-1)}(0) \\
&\qquad\qquad\qquad + \int_0^t\,\Xi\parn{s,\Gsoln\parn{\Thetabar^{(L-1)}(0),\Thetabar^{(L)}(0)}(s),\Thetabar^{(L)}(0),\Gsoln}\,ds.
\end{align*}
In other words, $\sT(\Gsoln)=\Gsoln$ a.s.. The Proposition implies that there exists a $R$-special function $\Gsoln=G_o$ a.e. , and this finishes the proof because it achieves Goal \ref{eq:goalspecialcontainssoln}.

We now prove the Claim. In what follows, we will use symbols $V_0,V_1,\dots$ to denote positive quantities that only depend on $C_{\ref{assump:activations}}$ and $L$.

To start, we observe that, although we do not know if $\soln_{[0,T]}$ is $R$-special, we have (\ref{eq:Gisusefulforsoln}). As a consequence, the reasoning in the proof of Lemma \ref{lem:redefiningzL} applies, with $\soln_{[0,T]}$ replacing $\nu_{[0,T]}$ and $\Gsoln$ replacing $F_\nu$. The upshot is that, for $P\times \mu_0^{(L)}$-a.e. $(x,a^{(L)})\in \R^{d_X}\times \R^{D_L}$, we have the following identity for all $t\in [0,T]$:
\[
\zbar^{(L)}\parn{x,\soln_t,a^{(L)}} =  \int\limits_{\R^{D_{L-1}}}\fsigma{L}{\zbar^{(L-1)}\parn{x,\soln_t)},\Gsoln\parn{\tilde{a}^{(L-1)},a^{(L)}}(t)}\,d(\soln_0)^{(L-1)}(\tilde{a}^{(L-1)}).
\]

Let us rewrite this as follows. Define $\Xi_0:[0,T]\times \R^{d_X}\times \R^{D_{L}}\times \sU$
via the following recipe: for $(t,x,a^{(L)},g)\in [0,T]\times \R^{d_X}\times \R^{D_{L}}\times \sU$,
\begin{equation}
\label{eq:defXi0}
\Xi_0\parn{t,x,a^{(L)},g}:=\int\limits_{\R^{D_{L-1}}}\fsigma{L}{\zbar^{(L-1)}\parn{x,\soln_t},g\parn{\tilde{a}^{(L-1)},a^{(L)}}(t)}\,d(\soln_0)^{(L-1)}(\tilde{a}^{(L-1)}).
\end{equation}

Then $\zbar^{(L)}\parn{x,\soln_t,a^{(L)}}=\Xi_0\parn{t,x,a^{(L)},\Gsoln}$ for every $(t,x)$ and $\mu_0^{(L-1)}$-almost-every $a^{(L)}$. Moreover, the map $\Xi_0$ satisfies analogues of the properties (1) - (5) in Proposition \ref{prop:Picardcomplicated}.

\begin{enumerate}
\item[(1')] $\Xi_0$ is bounded by $V_0$ because $\sigma^{(L-1)}$ is bounded by $C_{\ref{assump:activations}}$
\item[(2')] $\Xi_0\parn{t,x,a^{(L)},g_1}=\Xi_0\parn{t,x,a^{(L)},g_2}$ for $\mu_0^{(L)}$-almost everywhere  $a^{(L)}$ if $g_1=g_2$ $\quad\mu_0^{(L-1,L)}$-almost everywhere;
\item[(3')] for all $g\in\sU$, the map $(t,x,a^{(L)})\mapsto \Xi_0\parn{t,x,a^{(L)},g}$ is measurable for being a composition of measurable functions, and it is continuous in $t$ for similar reasons;
\item[(4')] Since $\supnorm{D\sigma^{(L)}}\leq C_{\ref{assump:activations}}$, then $\sigma^{(L)}$ is $C_{\ref{assump:activations}}$-Lipschitz. So
\begin{align*}
& \abs{\Xi_0\parn{t,x,a^{(L)},g} - \Xi_0\parn{t,x,b^{(L)},g}}\\
&\quad\quad\leq C_{\ref{assump:activations}}\,\int\limits_{\R^{D_{L-1}}}\abs{g\parn{\tilde{a}^{(L-1)},a^{(L)}}(t) - g\parn{\tilde{a}^{(L-1)},b^{(L)}}(t)}\,d(\soln)_0^{(L-1)}(\tilde{a}^{(L-1)})\\
&\quad\quad\leq  C_{\ref{assump:activations}}	\,\sup\limits_{\stackrel{a',b'\in\R^{D_{L-1}}\times \R^{D_L}}{\abs{a'-b'}\leq \epsilon}} \abs{g(a')(t)-g(b')(t)};
\end{align*}
\item[(5')] finally, for $g_1,g_2\in\sU$ and $(t,x,a^{(L)})$ as above, using again the Lipschitz property:
\[
\abs{\Xi_0\parn{t,a^{(L-1)},a^{(L)},g_1} - \Xi_0\parn{t,a^{(L-1)},a^{(L)},g_2}}\leq V_0\cdot\dist(g_1,g_2;t).
\]
\end{enumerate}

Going back to the Definition \ref{eq:defMbarL-Lminus1} for $\Mbar^{(L)}(x,\soln_t,a^{(L)})$, we see at once that we can define
\[
\Mbar^{(L)}(x,\soln_t,a^{(L)}) =: \Xi_1\parn{t,x,a^{(L)},\Gsoln}\mbox{ a.e.}
\]
where for $(t,x,a^{(L)},g)\in [0,T]\times \R^{d_X}\times \R^{D_L}\times \sU$:
\[
\Xi_1\parn{t,x,a^{(L)},g}:= \Mbar^{(L+1)}(x,\soln_t)\cdot D_z\fsigma{L}{\Xi_0\parn{t,x,a^{(L)},g},a^{(L)}}.
\]
$\Xi_1$ satisfies similar properties to (1')-(5') with a constant $V_1$ replacing $V_0$, because $\Mbar^{(L+1)}$ is bounded by $C_{\ref{assump:activations}}$ and $D_z\sigma^{(L)}$ is $C_{\ref{assump:activations}}$-Lipschitz.

The same is true (with a different constant $V_2$ replacing $V_1$) for the map
\[
\Xi_2\parn{t,x,a,g}:=\Xi_1\parn{t,x,a^{(L)},g}\cdot D_\theta\fsigma{L-1}{\zbar^{(L-1)}(x,\soln_t),a^{(L-1)}},
\]
defined for $(t,x,a,g)\in [0,T]\times \R^{d_X}\times(\R^{D_{L-1}}\times \R^{D_L})\times \sU$; the only change from the previous case is that we replace $a^{(L)}$ with $a$ where needed. Notice also that $\Xi_2$ satisfies:
\[
\Xi_2\parn{t,x,a,\Gsoln} = \Gamma({\bf a},x,\soln_t)\,
\]
for $\mu_0^{(L)}$-almost every choice of $a^{(L)}$ and all choices of ${\bf a}=(a^{(\ell)})_{\ell=0}^{L}$ extending $a^{(L)}$.

The conclusion is that the function
\[
\Xi(t,a,g):=\alpha(t)\,\Exp{(X,Y)\sim P}{(Y-\ybar(x,\soln_t))\,\Xi_2(t,X,a,g)},
\]
defined for $(t,a,g)\in [0,T]\times(\R^{D_{L-1}}\times \R^{D_L})\times \sU$ satisfies properties (1) - (5) in the statement of Proposition \ref{prop:Picardcomplicated}. Moreover
\[
\gbar^{(L-1)}({\bf a},\soln_t)= \Xi(t,a,\Gsoln)
\]
for $\mu_0^{(L)}$-a.e. choice of $a^{(L)}$ and all choices of ${\bf a}=(a^{(\ell)})_{\ell=0}^{L}$ extending $a^{(L)}$. By Lemma \ref{lem:constrainstructure}, we know that, if $\Thetabar\sim \psi(\soln_{[0,T]})=\soln_{[0,T]}$, then a.s. for all $t\geq 0$,
\[
\Thetabar^{(L-1)}(t) = \Thetabar^{(L-1)}(0) + \int_0^t\,\Xi\parn{s,\Thetabar^{(L-1)}(s),\Thetabar^{(L)}(0),\Gsoln}\,ds.
\]
This proves Claim \ref{claim:Xiexists}.
\end{proof}


==> measureNN_aux/A6-specialmeasures.tex <==
We prove here that the set $\Probspecial_R$ defined in \S \ref{sub:towardsfixedpoint} is closed under weak convergence.

\begin{proof}[Proof of Theorem \ref{thm:Probspecialisclosed}] Let $\Probspecial_R$ denote the set of $R$ special probability measures (cf. Definition \ref{def:Rspecialmeasure}). Consider a sequence $\{\mu_{j,[0,T]}\}_{j\in\N}\subset \Probspecial_R$. Each measure $\mu_j$ in the sequence has a corresponding $R$-special function $F_j:=F_{\mu_{j}}$, with the properties required by Definition \ref{def:Rspecialfunction}.

Assume that the sequence $\{\mu_{j,[0,T]}\}_{j\in\N}$ converges to some $\mu_{[0,T]}\in \Probspace(C([0,T],\R^D))$. We wish to show that $\mu_{[0,T]}\in\Probspecial_R$. The fact that $\mu_0$ is a product and the $L$-th coordinate is a.s. constant under $\mu_{[0,T]}$ are straightforward to show, and we omit them. The main point is to prove that there exists a special function $F=F_{\mu_{[0,T]}}$ (as per Definition \ref{def:Rspecialfunction}) which attests that $\mu$ is a special measure (as per Definition \ref{def:Rspecialmeasure}). To do this, we will use the following Claim.
\begin{claim}There exist a subsequence $\{j_k\}_{k\in\N}\subset \N$ a function $F:\R^{D_{L-1}}\times \R^{D_L}\to C([0,T],\R^{D_{L-1}})$ such that $F_{j_k}\to F$ uniformly over compact sets when $k\to +\infty$.\end{claim}

In what follows, we first show that the Claim implies that $\mu_{[0,T]}\in\Probspecial_R$, and then prove the Claim.

\underline{Proof that the Claim implies $\mu_{[0,T]}\in\Probspecial_R$.} By passing to a subsequence, we may assume that $F_j\to F$ uniformly over compact sets. We will use this to show that we may take $F_{\mu}:=F$ in Definition \ref{def:Rspecialmeasure} to certify that $\mu_{[0,T]}$ is $R$-special. 

To do this, we first argue that $F$ is $R$-special. This is simple: inspection of Definition \ref{def:Rspecialfunction} reveals that the properties required of a $R$-special functions are preserved under pointwise convergence, and thus also under uniform convergence over compact sets.

We now argue that $F$ attests that $\mu$ is $R$-special. That is, we will show that, if $\Theta\sim \mu_{[0,T]}$, then $\Theta_{[0,T]}^{(L-1)}=F(\Theta^{(L-1)}(0),\Theta^{(L)}(0))$ a.s.. 

The Skorohod representation theorem for weak convergence implies that we can find random elements $\Theta_{j,[0,T]}\sim \mu_{j}$ ($j\in \N$) and $\Theta_{[0,T]}\sim \mu$, defined over some common probability space, so that $\|\Theta_j - \Theta\|_\infty\to 0$ almost surely. This implies that:
\[(\Theta_j^{(L-1)}(0),\Theta_j^{(L)}(0),\Theta_{j,[0,T]}^{(L-1)})\to (\Theta^{(L-1)}(0),\Theta^{(L)}(0),\Theta^{(L-1)}_{[0,T]})\mbox { a.s.}.\]
Now, when $j\to +\infty$, the pair $(\Theta_j^{(L-1)(0)},\Theta_j^{(L)}(0))$ is a.s. convergent, so there a.s. is some (random) $R\in [0,+\infty)$ with: 
\[\sup_{j\in\N}|(\Theta_j^{(L-1)}(0) ,\Theta_j^{(L)}(0))|\leq R\mbox{ almost surely.}\]
This guarantees:
\begin{eqnarray*}& \limsup_j\|F_j(\Theta_j^{(L-1)}(0),\Theta_j^{(L)}(0)) -F(\Theta_j^{(L-1)}(0),\Theta_j^{(L)}(0))\|_{\infty}\\ \leq& (\limsup_j\sup_{|(a,b)|\leq R}\|F_j(a,b) - F(a,b)\|_{\infty})\\ =& 0\mbox{ a.s. because $F_j\to F$ uniformly over compact sets.}\end{eqnarray*}
For each $j\in\N$, we know that $F_j(\Theta_j^{(L-1)}(0),\Theta_j^{(L)}(0)) = \Theta^{(L-1)}_{j,[0,T]}$ a.s. for each $j\in\N$. This means we may replace $F_j(\Theta_j^{(L-1)}(0),\Theta_j^{(L)}(0))$ with $\Theta^{(L-1)}_{j,[0,T]}$ in the previous display and obtain:  
\[\|\Theta_{j,[0,T]}^{(L-1)} -F(\Theta_j^{(L-1)}(0),\Theta_j^{(L)}(0))\|_{\infty} \to 0\mbox{ a.s..}\]
Using continuity of $F$ and the convergence of $\Theta_j$, we obtain:
\[\|\Theta_{[0,T]}^{(L-1)} -F(\Theta^{(L-1)}(0),\Theta^{(L)}(0))\|_{\infty}=0\mbox{ a.s.},\]
which is what we wished to show.

\underline{Proof of the Claim.} We will need the following form of the Ascoli-Arz\`{e}la Theorem.

\begin{theorem}[Ascoli-Arz\`{e}la Theorem] Suppose $(X,\rho_X)$ and $(Y,\rho_Y)$ are metric spaces and $M>0$. Assume that all closed balls in $X$ are compact. Assume $\sH=\{f_j\}_{j\in\N}$ is a sequence of equicontinuous mappings $f:X\to Y$ such that the sets
\[\sH(x):=\{f_j(x)\,:\,j\in\N\}\;\;(x\in X)\]
are precompact\footnote{Recall that a set in a topological space is precompact if its closure is compact, or equivalently, if it is contained in a compact set.} subsets of $Y$. Then there exists a subsequence $\{f_{j_k}\}_{k\in\N}$ and a continuous function $f:X\to Y$ such that $f_{j_k}\to f$ uniformly over compact sets of $X$ when $k\to +\infty$.\end{theorem}

This follows from the usual formulation of Ascoli-Arz\`{e}la for the case when $X$ is itself compact. We omit the details.

To apply the above Theorem, we take $X=\R^{D_{L-1}}\times \R^{D_L}$, $Y=C([0,T],\R^{D_{\ell-1}})$ and $\sH=\{F_j\}_{j\in\N}$. In order to deduce the Claim, we need to show that $\sH$ is equicontinous and that $\sH(x)$ is precompact for each $x\in X$.

We first show that $\sH$ is equicontinuous. Note that, if $a,b\in \R^{D_{L-1}}\times \R^{D_{L}}$ and $t\in [0,T]$, property 1 in the definition of special measure implies:
\[\|F_j(a) - F_j(b)\|_{\infty} = \sup_{0\leq t\leq T}|F_j(a)(t) - F_j(b)(t)|\leq \sup_{0\leq t\leq T}e^{Rt}|a-b|\leq e^{RT}|a-b|.\]
In particular, all $F_j$ are $e^{RT}$-Lipschitz mappings from the set $\R^{D_{L-1}}\times \R^{D_{L}}$ to $C([0,T],\R^{D_{L-1}})$.

To check precompactness of the images $\sH(x)$, we use Property 2 of Definition \ref{def:Rspecialmeasure}, which ensures that, for each $x=(\theta^{(L-1)}(0),\theta^{(L)}(0))\in \R^{D_{L-1}}\times \R^{D_L}$,
\[\sH(x)\subset U(x):=\{f\in C([0,T],\R^{D_{\ell-1}})\,:\, f(0) = \theta^{(L-1)}(0)\mbox{ and }f\mbox{ is $R$-Lipschitz.}\}.\]
The set $U(x)$ is a closed subset of $C([0,T],\R^{D_{\ell-1}})$ that consists of uniformly bounded and equicontinuous functions. Since $[0,T]$ is compact,  the Ascoli-Arz\`{e}la theorem in its classical form guarantees that $U(x)$ is a compact subset of $Y=C([0,T],\R^{D_{\ell-1}})$. This implies that $\sH(x)$ is precompact, which finishes the proof of the claim.\end{proof}
